Sharp asymptotics on the compression of two-layer neural networks

In this paper, we study the compression of a target two-layer neural network with N nodes into a compressed network with M<N nodes. More precisely, we consider the setting in which the weights of the target network are i.i.d. sub-Gaussian, and we minimize the population L_2 loss between the outputs of the target and of the compressed network, under the assumption of Gaussian inputs. By using tools from high-dimensional probability, we show that this non-convex problem can be simplified when the target network is sufficiently over-parameterized, and provide the error rate of this approximation as a function of the input dimension and N. In this mean-field limit, the simplified objective, as well as the optimal weights of the compressed network, does not depend on the realization of the target network, but only on expected scaling factors. Furthermore, for networks with ReLU activation, we conjecture that the optimum of the simplified optimization problem is achieved by taking weights on the Equiangular Tight Frame (ETF), while the scaling of the weights and the orientation of the ETF depend on the parameters of the target network. Numerical evidence is provided to support this conjecture.

==> data/data_avg_M=10.tex <==
0	5.256171421
1	5.302321843
2	5.344110064
3	5.38179708
4	5.415703175
5	5.446175908
6	5.473565286
7	5.498206921
8	5.520412089
9	5.540462953
10	5.559927962
11	5.576280887
12	5.591162726
13	5.60474204
14	5.617165902
15	5.628562591
16	5.639044073
17	5.648708214
18	5.657640713
19	5.665916782
20	5.673602578
21	5.680756437
22	5.687429917
23	5.693668698
24	5.699513336
25	5.704999925
26	5.710160648
27	5.71502426
28	5.719616504
29	5.723960463
30	5.728076876
31	5.731984402
32	5.735699857
33	5.739238418
34	5.742613805
35	5.745838437
36	5.748923568
37	5.751879415
38	5.754715262
39	5.757439558
40	5.760060001
41	5.762583612
42	5.765016806
43	5.767365447
44	5.769634907
45	5.771830107
46	5.773955565
47	5.776015432
48	5.778013525
49	5.77995336
50	5.78183818
51	5.783670976
52	5.785454514
53	5.787191349
54	5.788883853
55	5.790534219
56	5.792144486
57	5.793716548
58	5.795252166
59	5.796752979
60	5.798220517
61	5.799656205
62	5.801061376
63	5.802437274
64	5.803785067
65	5.805105845
66	5.806400633
67	5.807670393
68	5.808916028
69	5.810138389
70	5.811338275
71	5.812516442
72	5.813673602
73	5.814810426
74	5.81592755
75	5.817025576
76	5.818105073
77	5.819166581
78	5.820210613
79	5.821237656
80	5.822248174
81	5.823242606
82	5.824221374
83	5.825184877
84	5.826133498
85	5.827067603
86	5.827987541
87	5.828893647
88	5.829786242
89	5.830665633
90	5.831532117
91	5.832385977
92	5.833227487
93	5.83405691
94	5.834874499
95	5.8356805
96	5.836475149
97	5.837258674
98	5.838031296
99	5.83879323
100	5.839544683
101	5.840285855
102	5.841016942
103	5.841738134
104	5.842449614
105	5.843151563
106	5.843844155
107	5.84452756
108	5.845201943
109	5.845867467
110	5.846524289
111	5.847172563
112	5.84781244
113	5.848444067
114	5.849067588
115	5.849683145
116	5.850290875
117	5.850890913
118	5.851483393
119	5.852068443
120	5.852646191
121	5.853216761
122	5.853780278
123	5.85433686
124	5.854886626
125	5.855429692
126	5.855966171
127	5.856496175
128	5.857019814
129	5.857537197
130	5.858048428
131	5.858553612
132	5.859052852
133	5.859546248
134	5.860033899
135	5.860515902
136	5.860992353
137	5.861463345
138	5.861928971
139	5.862389321
140	5.862844485
141	5.86329455
142	5.863739601
143	5.864179724
144	5.864615002
145	5.865045515
146	5.865471344
147	5.865892568
148	5.866309264
149	5.866721507
150	5.867129373
151	5.867532933
152	5.867932261
153	5.868327425
154	5.868718496
155	5.86910554
156	5.869488624
157	5.869867813
158	5.870243172
159	5.870614762
160	5.870982644
161	5.87134688
162	5.871707527
163	5.872064644
164	5.872418286
165	5.87276851
166	5.873115369
167	5.873458916
168	5.873799203
169	5.874136281
170	5.874470199
171	5.874801007
172	5.875128751
173	5.875453479
174	5.875775235
175	5.876094064
176	5.87641001
177	5.876723115
178	5.87703342
179	5.877340967
180	5.877645794
181	5.87794794
182	5.878247444
183	5.878544343
184	5.878838671
185	5.879130466
186	5.87941976
187	5.879706589
188	5.879990983
189	5.880272977
190	5.880552601
191	5.880829885
192	5.881104859
193	5.881377554
194	5.881647996
195	5.881916214
196	5.882182234
197	5.882446085
198	5.88270779
199	5.882967375
200	5.883224866
201	5.883480285
202	5.883733657
203	5.883985004
204	5.884234349
205	5.884481713
206	5.884727117
207	5.884970583
208	5.885212131
209	5.885451781
210	5.885689551
211	5.885925461
212	5.886159529
213	5.886391773
214	5.886622211
215	5.886850859
216	5.887077736
217	5.887302856
218	5.887526236
219	5.887747892
220	5.887967838
221	5.88818609
222	5.888402663
223	5.88861757
224	5.888830825
225	5.889042442
226	5.889252434
227	5.889460814
228	5.889667594
229	5.889872788
230	5.890076407
231	5.890278463
232	5.890478967
233	5.890677931
234	5.890875366
235	5.891071282
236	5.89126569
237	5.891458601
238	5.891650024
239	5.891839969
240	5.892028446
241	5.892215465
242	5.892401034
243	5.892585162
244	5.892767859
245	5.892949132
246	5.893128991
247	5.893307443
248	5.893484497
249	5.893660161
250	5.893834441
251	5.894007347
252	5.894178885
253	5.894349062
254	5.894517886
255	5.894685363
256	5.894851501
257	5.895016306
258	5.895179784
259	5.895341943
260	5.895502788
261	5.895662325
262	5.895820561
263	5.895977502
264	5.896133154
265	5.896287522
266	5.896440612
267	5.89659243
268	5.89674298
269	5.89689227
270	5.897040303
271	5.897187086
272	5.897332623
273	5.897476919
274	5.89761998
275	5.897761811
276	5.897902417
277	5.898041802
278	5.898179972
279	5.898316931
280	5.898452685
281	5.898587237
282	5.898720593
283	5.898852757
284	5.898983734
285	5.899113529
286	5.899242147
287	5.899369591
288	5.899495868
289	5.89962098
290	5.899744934
291	5.899867733
292	5.899989382
293	5.900109886
294	5.90022925
295	5.900347478
296	5.900464575
297	5.900580545
298	5.900695394
299	5.900809126
300	5.900921745
301	5.901033258
302	5.901143667
303	5.901252979
304	5.901361199
305	5.90146833
306	5.901574379
307	5.901679349
308	5.901783248
309	5.901886078
310	5.901987846
311	5.902088556
312	5.902188215
313	5.902286827
314	5.902384397
315	5.902480932
316	5.902576436
317	5.902670915
318	5.902764374
319	5.90285682
320	5.902948257
321	5.903038692
322	5.903128131
323	5.903216579
324	5.903304042
325	5.903390526
326	5.903476037
327	5.903560582
328	5.903644166
329	5.903726795
330	5.903808477
331	5.903889216
332	5.903969021
333	5.904047896
334	5.904125849
335	5.904202886
336	5.904279014
337	5.904354239
338	5.904428568
339	5.904502008
340	5.904574566
341	5.904646248
342	5.904717063
343	5.904787015
344	5.904856113
345	5.904924364
346	5.904991775
347	5.905058352
348	5.905124104
349	5.905189037
350	5.905253159
351	5.905316478
352	5.905378999
353	5.905440732
354	5.905501683
355	5.90556186
356	5.905621271
357	5.905679923
358	5.905737823
359	5.90579498
360	5.905851401
361	5.905907093
362	5.905962065
363	5.906016324
364	5.906069878
365	5.906122735
366	5.906174902
367	5.906226387
368	5.906277198
369	5.906327344
370	5.906376831
371	5.906425668
372	5.906473862
373	5.906521422
374	5.906568355
375	5.906614669
376	5.906660373
377	5.906705473
378	5.906749978
379	5.906793896
380	5.906837235
381	5.906880002
382	5.906922205
383	5.906963852
384	5.907004952
385	5.907045511
386	5.907085538
387	5.90712504
388	5.907164025
389	5.907202502
390	5.907240476
391	5.907277957
392	5.907314953
393	5.907351469
394	5.907387515
395	5.907423098
396	5.907458225
397	5.907492904
398	5.907527142
399	5.907560948
400	5.907594327
401	5.907627288
402	5.907659838
403	5.907691984
404	5.907723734
405	5.907755094
406	5.907786073
407	5.907816676
408	5.907846911
409	5.907876786
410	5.907906306
411	5.90793548
412	5.907964313
413	5.907992814
414	5.908020987
415	5.908048841
416	5.908076382
417	5.908103616
418	5.90813055
419	5.90815719
420	5.908183544
421	5.908209617
422	5.908235416
423	5.908260946
424	5.908286215
425	5.908311228
426	5.908335991
427	5.908360511
428	5.908384793
429	5.908408843
430	5.908432667
431	5.908456271
432	5.90847966
433	5.908502841
434	5.908525818
435	5.908548597
436	5.908571184
437	5.908593584
438	5.908615803
439	5.908637845
440	5.908659715
441	5.90868142
442	5.908702963
443	5.90872435
444	5.908745585
445	5.908766675
446	5.908787622
447	5.908808433
448	5.908829111
449	5.908849661
450	5.908870087
451	5.908890395
452	5.908910588
453	5.908930671
454	5.908950648
455	5.908970522
456	5.908990299
457	5.909009982
458	5.909029574
459	5.909049081
460	5.909068505
461	5.90908785
462	5.909107121
463	5.909126319
464	5.90914545
465	5.909164517
466	5.909183522
467	5.909202469
468	5.909221362
469	5.909240203
470	5.909258996
471	5.909277743
472	5.909296448
473	5.909315113
474	5.909333742
475	5.909352336
476	5.909370899
477	5.909389434
478	5.909407942
479	5.909426426
480	5.909444889
481	5.909463333
482	5.90948176
483	5.909500173
484	5.909518573
485	5.909536962
486	5.909555343
487	5.909573718
488	5.909592087
489	5.909610454
490	5.909628819
491	5.909647185
492	5.909665553
493	5.909683924
494	5.9097023
495	5.909720682
496	5.909739072
497	5.90975747
498	5.909775878
499	5.909794298
500	5.909812729
501	5.909831174
502	5.909849632
503	5.909868105
504	5.909886594
505	5.909905098
506	5.90992362
507	5.909942159
508	5.909960716
509	5.909979291
510	5.909997885
511	5.910016498
512	5.91003513
513	5.910053782
514	5.910072453
515	5.910091144
516	5.910109855
517	5.910128585
518	5.910147335
519	5.910166104
520	5.910184892
521	5.910203699
522	5.910222525
523	5.910241368
524	5.910260229
525	5.910279107
526	5.910298001
527	5.910316911
528	5.910335836
529	5.910354776
530	5.910373728
531	5.910392694
532	5.910411671
533	5.910430659
534	5.910449657
535	5.910468664
536	5.910487678
537	5.910506698
538	5.910525724
539	5.910544754
540	5.910563786
541	5.91058282
542	5.910601854
543	5.910620886
544	5.910639915
545	5.91065894
546	5.910677959
547	5.910696971
548	5.910715973
549	5.910734965
550	5.910753944
551	5.910772909
552	5.910791858
553	5.910810789
554	5.910829701
555	5.910848592
556	5.910867459
557	5.910886301
558	5.910905116
559	5.910923903
560	5.910942658
561	5.910961381
562	5.910980069
563	5.910998721
564	5.911017333
565	5.911035905
566	5.911054434
567	5.911072918
568	5.911091356
569	5.911109744
570	5.911128082
571	5.911146366
572	5.911164595
573	5.911182768
574	5.911200881
575	5.911218932
576	5.911236921
577	5.911254844
578	5.911272699
579	5.911290485
580	5.9113082
581	5.911325841
582	5.911343407
583	5.911360895
584	5.911378304
585	5.911395632
586	5.911412876
587	5.911430035
588	5.911447107
589	5.91146409
590	5.911480982
591	5.911497782
592	5.911514487
593	5.911531097
594	5.911547608
595	5.91156402
596	5.91158033
597	5.911596538
598	5.911612641
599	5.911628639
600	5.911644528
601	5.911660309
602	5.911675979
603	5.911691537
604	5.911706982
605	5.911722312
606	5.911737527
607	5.911752624
608	5.911767602
609	5.911782461
610	5.911797199
611	5.911811816
612	5.911826309
613	5.911840679
614	5.911854924
615	5.911869043
616	5.911883035
617	5.9118969
618	5.911910637
619	5.911924245
620	5.911937723
621	5.911951071
622	5.911964288
623	5.911977373
624	5.911990327
625	5.912003148
626	5.912015837
627	5.912028392
628	5.912040814
629	5.912053102
630	5.912065256
631	5.912077275
632	5.912089161
633	5.912100912
634	5.912112528
635	5.912124011
636	5.912135358
637	5.912146571
638	5.91215765
639	5.912168595
640	5.912179406
641	5.912190083
642	5.912200626
643	5.912211037
644	5.912221314
645	5.912231459
646	5.912241473
647	5.912251354
648	5.912261105
649	5.912270725
650	5.912280215
651	5.912289575
652	5.912298807
653	5.912307911
654	5.912316887
655	5.912325736
656	5.91233446
657	5.912343058
658	5.912351531
659	5.912359881
660	5.912368108
661	5.912376213
662	5.912384196
663	5.91239206
664	5.912399804
665	5.91240743
666	5.912414938
667	5.91242233
668	5.912429606
669	5.912436768
670	5.912443817
671	5.912450753
672	5.912457578
673	5.912464293
674	5.912470898
675	5.912477395
676	5.912483786
677	5.91249007
678	5.91249625
679	5.912502326
680	5.912508299
681	5.912514171
682	5.912519943
683	5.912525616
684	5.912531191
685	5.912536669
686	5.912542052
687	5.91254734
688	5.912552535
689	5.912557638
690	5.91256265
691	5.912567572
692	5.912572406
693	5.912577152
694	5.912581812
695	5.912586387
696	5.912590878
697	5.912595286
698	5.912599613
699	5.912603859
700	5.912608026
701	5.912612115
702	5.912616127
703	5.912620063
704	5.912623925
705	5.912627712
706	5.912631428
707	5.912635072
708	5.912638645
709	5.91264215
710	5.912645586
711	5.912648955
712	5.912652258
713	5.912655497
714	5.912658671
715	5.912661783
716	5.912664833
717	5.912667822
718	5.912670751
719	5.912673622
720	5.912676435
721	5.912679191
722	5.912681891
723	5.912684537
724	5.912687128
725	5.912689667
726	5.912692153
727	5.912694589
728	5.912696974
729	5.91269931
730	5.912701598
731	5.912703838
732	5.912706031
733	5.912708179
734	5.912710281
735	5.91271234
736	5.912714355
737	5.912716327
738	5.912718258
739	5.912720148
740	5.912721997
741	5.912723808
742	5.912725579
743	5.912727313
744	5.912729009
745	5.912730669
746	5.912732294
747	5.912733883
748	5.912735438
749	5.912736959
750	5.912738447
751	5.912739902
752	5.912741326
753	5.912742719
754	5.912744081
755	5.912745414
756	5.912746717
757	5.912747991
758	5.912749237
759	5.912750456
760	5.912751648
761	5.912752813
762	5.912753953
763	5.912755067
764	5.912756156
765	5.912757221
766	5.912758262
767	5.91275928
768	5.912760275
769	5.912761248
770	5.912762198
771	5.912763128
772	5.912764036
773	5.912764924
774	5.912765792
775	5.91276664
776	5.912767469
777	5.912768279
778	5.91276907
779	5.912769844
780	5.9127706
781	5.912771339
782	5.912772061
783	5.912772766
784	5.912773455
785	5.912774128
786	5.912774786
787	5.912775429
788	5.912776057
789	5.91277667
790	5.91277727
791	5.912777855
792	5.912778427
793	5.912778986
794	5.912779532
795	5.912780065
796	5.912780585
797	5.912781094
798	5.912781591
799	5.912782076
800	5.91278255
801	5.912783013
802	5.912783465
803	5.912783906
804	5.912784337
805	5.912784759
806	5.91278517
807	5.912785571
808	5.912785963
809	5.912786346
810	5.91278672
811	5.912787085
812	5.912787442
813	5.91278779
814	5.91278813
815	5.912788462
816	5.912788786
817	5.912789102
818	5.912789411
819	5.912789713
820	5.912790007
821	5.912790295
822	5.912790575
823	5.912790849
824	5.912791117
825	5.912791378
826	5.912791633
827	5.912791882
828	5.912792125
829	5.912792362
830	5.912792593
831	5.912792819
832	5.91279304
833	5.912793255
834	5.912793465
835	5.912793671
836	5.912793871
837	5.912794066
838	5.912794257
839	5.912794443
840	5.912794625
841	5.912794802
842	5.912794975
843	5.912795144
844	5.912795309
845	5.91279547
846	5.912795627
847	5.912795781
848	5.91279593
849	5.912796076
850	5.912796219
851	5.912796358
852	5.912796494
853	5.912796626
854	5.912796755
855	5.912796881
856	5.912797004
857	5.912797125
858	5.912797242
859	5.912797356
860	5.912797468
861	5.912797577
862	5.912797683
863	5.912797787
864	5.912797888
865	5.912797986
866	5.912798083
867	5.912798177
868	5.912798269
869	5.912798358
870	5.912798445
871	5.912798531
872	5.912798614
873	5.912798695
874	5.912798774
875	5.912798851
876	5.912798927
877	5.912799
878	5.912799072
879	5.912799142
880	5.91279921
881	5.912799277
882	5.912799342
883	5.912799405
884	5.912799467
885	5.912799527
886	5.912799586
887	5.912799644
888	5.9127997
889	5.912799754
890	5.912799808
891	5.91279986
892	5.91279991
893	5.91279996
894	5.912800008
895	5.912800055
896	5.912800101
897	5.912800146
898	5.91280019
899	5.912800233
900	5.912800274
901	5.912800315
902	5.912800355
903	5.912800393
904	5.912800431
905	5.912800468
906	5.912800504
907	5.912800539
908	5.912800573
909	5.912800606
910	5.912800639
911	5.91280067
912	5.912800701
913	5.912800731
914	5.912800761
915	5.912800789
916	5.912800817
917	5.912800845
918	5.912800871
919	5.912800897
920	5.912800923
921	5.912800947
922	5.912800972
923	5.912800995
924	5.912801018
925	5.91280104
926	5.912801062
927	5.912801084
928	5.912801104
929	5.912801125
930	5.912801144
931	5.912801164
932	5.912801182
933	5.912801201
934	5.912801219
935	5.912801236
936	5.912801253
937	5.91280127
938	5.912801286
939	5.912801302
940	5.912801317
941	5.912801332
942	5.912801347
943	5.912801361
944	5.912801375
945	5.912801389
946	5.912801402
947	5.912801415
948	5.912801427
949	5.91280144
950	5.912801452
951	5.912801463
952	5.912801475
953	5.912801486
954	5.912801497
955	5.912801507
956	5.912801518
957	5.912801528
958	5.912801538
959	5.912801547
960	5.912801557
961	5.912801566
962	5.912801575
963	5.912801583
964	5.912801592
965	5.9128016
966	5.912801608
967	5.912801616
968	5.912801623
969	5.912801631
970	5.912801638
971	5.912801645
972	5.912801652
973	5.912801659
974	5.912801666
975	5.912801672
976	5.912801678
977	5.912801684
978	5.91280169
979	5.912801696
980	5.912801702
981	5.912801707
982	5.912801713
983	5.912801718
984	5.912801723
985	5.912801728
986	5.912801733
987	5.912801738
988	5.912801742
989	5.912801747
990	5.912801751
991	5.912801756
992	5.91280176
993	5.912801764
994	5.912801768
995	5.912801772
996	5.912801775
997	5.912801779
998	5.912801783
999	5.912801769
	


==> data/data_error_plot.tex <==
m                   min                 avg                 max
4.00000000000000	5.30331739084252	5.30331739084252	5.30331739084252
5.00000000000000	5.51499122826825	5.51499122826825	5.51499122826825
6.00000000000000	5.65108021380762	5.65108021380762	5.65108021380762
7.00000000000000	5.74607107836515	5.74607181944627	5.74607190178953
8.00000000000000	5.74591545957013	5.80283158362687	5.81618415978184
9.00000000000000	5.81589583659655	5.86331381971036	5.87007664699325
10.00000000000000	5.87075660207135	5.90859737757146	5.91280192459169
15.00000000000000	6.03645948868461	6.03867675990636	6.03899688175824
20.00000000000000	6.09136676249814	6.09927032546893	6.10089441525132
30.00000000000000	6.15688878459893	6.15810748582212	6.15915381588203


